Fix your classifier: the marginal value of training the last weight layer

Neural networks are commonly used as models for classification for a wide variety of tasks. Typically, a learned affine transformation is placed at the end of such models, yielding a per-class value used for classification. This classifier can have a vast number of parameters, which grows linearly with the number of possible classes, thus requiring increasingly more resources. In this work we argue that this classifier can be fixed, up to a global scale constant, with little or no loss of accuracy for most tasks, allowing memory and computational benefits. Moreover, we show that by initializing the classifier with a Hadamard matrix we can speed up inference as well. We discuss the implications for current understanding of neural network models.

==> max_margin.tex <==
Our findings suggest that common practices used may be misguided. For example, several works (e.g \cite{he2016deep}) suggested to decrease learning rate when the validation error plateaus. This practice is even advocated and automated by widely used frameworks such as Keras, Pytorch. 
Instead, we highlight the fact that final validation accuracy may benefit from prolonged training with a high learning rate, even without noticeable improvement in the short range. 

We also note the possible negative impact of weight decay, especially at late stages of training, where it may hurt the logarithmic growth needed to reach a maximum margin solution.


Keras: https://keras.io/callbacks/#reducelronplateau
pytorch: http://pytorch.org/docs/master/optim.html#how-to-adjust-learning-rate

==> rebuttal.tex <==
AnonReviewer1:

We thank the reviewer for his detailed feedback on our paper.
We hope to address the 2 main concerns raised:
1) Novelty - "removing the fully connected classification layer is not a novel idea; All Convolutional Networks (https://arxiv.org/abs/1412.6806) reported excellent results without an additional fully connected affine transform (just a global average pooling after the last convolutional layer)"

We believe there is a slight misunderstanding here: in the "All convolutional networks" paper the fully-connected was not removed, as it just got replaced with a convolutional layer with the same number of parameters. This means there is still a final classifier (a conv layer) with number of parameters proportional to the number of classes.
Our work introduces what we believe to be a novel idea - removing the classifier layer altogether making the number of network parameters independent from the number of classes. We added a clarification to this matter in our recent revision. 

2) Applicability of our method when C > N:

The reviewer is right in his claim that when C > N we can not have mutually orthogonal columns, but this is true even for a fully learned weight matrix. 
We empirically verified that for the vision use-cases brought in the paper we achieve good performance for C > N (e.g., on imagenet, so C=1000, with either mobilenet 0.5 where N = 512 or resnet with N reduced to 256).
We do agree with the reviewer that this can be limiting when the classes have strong correlation with one another (as in the NLP case) and we add this as another possible explanation. We still, however, feel that this can be useful even for C >> N in other domains such as vision.


AnonReviewer2:
We thank the reviewer for his feedback and suggestions. We added an explanation as well as extended the supplementary code for the case where number of penultimate features does not match the number of classes.
We also added to the discussion the case where C >> N. Regarding distillation - we found no apparent difference when distilling a network with fixed classifier.

AnnonReviewr3:
We thank the reviewer for his detailed feedback on our paper and his suggestions. We hope to answer his questions below. We also made adjustments to latest revision accordingly.

1) "Are the scale and bias regularized?" - Yes. We found that regularization can help with the final validation error in the same way it helps with common learned weights. Best results appeared when trained with weight decay for several epochs and removed later.

2) "how does the chosen projection matrix affect performance" - We found no significance change in final accuracy when using different projection matrix. We do find slight change in convergence rate when initial scale is changed.

3) "is the scale needed" - We added some experiments to show that the scale is not needed as a learned parameter, but this may help convergence.

4) "The amount of computation saved seems rather limited?" - The compute saved is for the gradient of the classifier weights (which is not needed to get the gradient for the scale). This may be limited for the cases shown, but becomes more apparent when number of classes is larger. As we noted, these gradients and weights can now be avoided in communication over several nodes in distributed setting - saving precious bandwidth. Moreover using a Hadamard matrix we can replace all multiplication operations preformed by the classifier with additions which are far more hardware friendly. 

5)"Is there an intuition why the training error remains higher but the validation error is identical?" - Our conjecture is that with our new fixed parameterization, the network can no longer increase the norm of a given sample's representation - thus learning its label requires more effort. As this may happen for specific seen samples - it affects only training error.

Regarding clarity and manuscript structure - we have taken the reviewer's comments into account and revised our paper accordingly.


